Echoes Beyond Points: Unleashing the Power of Raw Radar Data in Multi-modality Fusion

Radar is ubiquitous in autonomous driving systems due to its low cost and good adaptability to bad weather. Nevertheless, the radar detection performance is usually inferior because its point cloud is sparse and not accurate due to the poor azimuth and elevation resolution. Moreover, point cloud generation algorithms already drop weak signals to reduce the false targets which may be suboptimal for the use of deep fusion. In this paper, we propose a novel method named EchoFusion to skip the existing radar signal processing pipeline and then incorporate the radar raw data with other sensors. Specifically, we first generate the Bird's Eye View (BEV) queries and then take corresponding spectrum features from radar to fuse with other sensors. By this approach, our method could utilize both rich and lossless distance and speed clues from radar echoes and rich semantic clues from images, making our method surpass all existing methods on the RADIal dataset, and approach the performance of LiDAR. The code will be released on https://github.com/tusen-ai/EchoFusion.

==> Sections/2_related_works.tex <==
\section{Related Works}
\subsection{Deep Learning on Radar}
\subsubsection{Radar Data Representation and Datasets}
Traditional radar usually only outputs sparse points\cite{schumann2021radarscenes, deziel2021pixset,caesar2020nuscenes} for use. However, such points are subjective to heavy signal processing methods to reduce noisy observation and alleviate bandwidth limitation. Nevertheless, such hand-crafted pipeline makes subsequent fusion with other sensors intractable. Consequently, some attempts have been made to provide upstream data, such as range-azimuth-Doppler (RAD) tensor \cite{ouaknine2021carrada,zhang2021raddet}, range-azimuth (RA) maps \cite{sheeny2021radiate}, range-Doppler (RD) spectrums \cite{mostajabi2020high} or even raw Analog Digital Converter (ADC) 
 data\cite{lim2021radical}\cite{mostajabi2020high}. Note that the RAD, RA and RD map are generated from ADC data using several times of (almost) lossless FFT. Thus we call these all these four types of data ``radar raw data" in the sequel.

%Radar point cloud  and the  are the most prevalent formats for their fully decoded off-the-shelf attributes. The low transmission bandwidth requirement and light representation of radar point cloud make it extremely suitable for multi-modality datasets of numerous amounts such as nuScenes \cite{}. Other datasets provide as radar data formats. 


\begin{table}
  \caption{4D Radar Datasets Comparison. Data: PC, RA, ADC denote to point cloud, range azimuth map and raw ADC data; Sensors: C, $C_s$, L, O denote to camera, stereo camera, LiDAR and odometer; Scenarios: U, S, H denote to urban (city), suburban, highway; Annotations: 3D, BEV, T, $P_o$, M denote to 3D bounding box, BEV bounding box, track ID, object-level point and segmentation mask; Classes and Size denote the number of classes and number of annotated frames of each dataset.}
  \label{dataset}
  \centering
  \begin{tabular}{lllllll}
    \toprule
    Dataset & Data & Other Sensors & Scenarios & Annotations & Classes & Size \\
    \midrule
    Astyx \cite{meyer2019automotive} & PC & CL & SH & 3D & 7 & 500 \\
    View-of-Delft \cite{palffy2022multi} & PC & $C_s$LO & U & 3D,T & 13 & 8693 \\
    RADIal \cite{rebut2022raw} & ADC,RA,PC & CLO & USH & $P_o$,M & 1 & 8252 \\
    TJ4DRadSet \cite{zheng2022tj4dradset} & PC & CLO & U & 3D,T & 5 & 7757 \\
    Radatron \cite{madani2022radatron} & ADC,RA & $C_s$ & U & BEV & 1 & 16K \\
    \bottomrule
  \end{tabular}
\end{table}

%By using large arrays of virtual antennas, 4D radars successfully alleviate sparsity and low angular resolution problems of traditional ones. Several datasets have recently been released for detection tasks on 4D radar data, as shown in Table \ref{dataset}. As can be observed, most datasets provide point cloud as the only radar data format \cite{meyer2019automotive}\cite{palffy2022multi}\cite{zheng2022tj4dradset}, which leads to information loss and super sparsity at the input side. 
Since our motivation is to deeply fuse with other sensors, we only consider the datasets providing data beyond point cloud. Among them, both RADIal \cite{rebut2022raw} and Radatron \cite{madani2022radatron} provide such data. But the latter one only covers a single scenario while lacking camera calibration, LiDAR modality, and vertical\footnote{height?} annotation. Taking into account the factors mentioned above, we carried out all our experiments on the RADIal dataset. However, the annotations of RADIal only contain object-level points. For a more comprehensive and objective evaluation, we further annotate the bounding box size and heading of each object based on dense LiDAR points. The annotations will be released to the community soon. 


\subsubsection{Object Detection on Radar Data}
Traditional radar object detection method that utilizes point cloud faces challenges of super sparsity due to the low angular resolution. Practical treatments include occupancy grid mapping \cite{zhou2022towards} and separate processing for static and dynamic objects \cite{schumann2019scene}. 4D radar technology improves the azimuth resolution and provide additional elevation resolution, which enables the combination of static and dynamic object detection in a single network, using either PointPillars \cite{palffy2022multi} or tailor-made self-attention modules \cite{xu2021rpfa}\cite{bai2021radar}.

The pre-CFAR(Constant False Alarm Rate Detector) data provide rich information of both targets and backgrounds. RAD tensor is fully decoded but brings high demand of storage and computation. Hence, Zhang et al. \cite{zhang2021raddet} takes the Doppler dimension as channels and Major et al. \cite{major2019vehicle} projects RAD tensor to multiple 2D views. RTCNet \cite{palffy2020cnn} divides RAD tensor into small cubes and applies 3D CNN to reduce computation burden. Besides, \cite{zhang2020object}\cite{rebut2022raw} take complex RD spectrum as input and apply neural networks to automatically extract spatial information. Networks such as RODNet \cite{wang2021rodnet} adopt complex RA maps for detection, which avoid false alarms caused by extended Doppler proﬁle.


The fusion of different sensors provides complementary cues, leading to more robust performance. At input level, radar point clouds are usually projected as pseudo-images and concatenated with camera images \cite{nobis2019deep}\cite{chadwick2019distant}. At Region of Interest (RoI) level, the RoIs are either consecutively refined by radar and other modalities \cite{nabati2020radar}\cite{nabati2021centerfusion} or unified together from different sensors \cite{kim2020grif}\cite{kim2023crn}.\footnote{not clear. need rewrite.} At feature level, 
\cite{wu2023mvfusion}\cite{zhang2021rvdet} integrates feature maps generated from different modalities, while \cite{kim2020low}\cite{kim2022craft} use RoIs to crop and merge features across modalities. To the best of our knowledge, we are the first to deeply fuse radar using raw data with other modalities in a unified BEV perspective. %we are not only the first method that utilizes BEV queries to extract features from different modalities, but also the first to take radar data only processed by range FFT as inputs. 


\subsection{BEV 3D Object Detector}\footnote{need cite more papers like bevdepth, bevstereo, bevfusion, petrv2, etc...}
% 按照LSS正投影，query反投影
% 多模态融合，其他信息（时序，depth监督）
% 这几个角度和逻辑重新写一下覅吧
BEV object detection bursts out a rising wave of research due to its vast success in 3D perception tasks. OFT \cite{roddick2018orthographic} and VPN \cite{pan2020cross} are the first literature that project single-view and multi-view images to BEV space for 3D scene understanding, respectively. Modern BEV-based algorithms benefit from the increase of available multi-sensor data. CVT \cite{zhou2022cross} merges perspective view and BEV features by applying camera-aware positional embedding and attention mechanism. PETR \cite{liu2022petr} projects image features to 3D embedded space, which is further processed by DETR-style decoders. BEVFormer \cite{li2022bevformer} and its variant \cite{yang2022bevformer} use BEV representation to fuse both spatial and temporal information from multiple perspectives. Furthermore, simpleBEV \cite{harley2022simple} introduces a deformable multi-scale BEV fusion mechanism while BEVDet \cite{huang2021bevdet} explores image-level and BEV-level augmentation strategies. As fully transformer-based structures free BEV detectors from uniform and regular sampling grids, PolarFormer \cite{jiang2022polarformer} realizes multi-view image fusion under polar coordinates. Considering the natural polar structure of both radar and image data and  the versatile fusion ability of attention, we choose PolarFormer as our stem structure. What makes our method different is our concentration on single-view multi-modalities fusion and specifically designed attention mechanisms for sensors with different properties.

==> Sections/3_method.tex <==
\section{Preliminary}
\label{preliminary}
% If an object with radial speed $v$ has a radial distance $R_0$ and angle of arrival (AoA) $\theta$ to the radar, it will have a complex response on ADC data with phase:
% \begin{equation}
%     \label{phase}
%     \begin{aligned}
%         &P_{D}^{H}\left( \mathrm{m},\mathrm{n},\mathrm{k} \right) \approx 2\pi \left[ -\mu \cdot \tau _0\cdot \mathrm{m}\cdot T_s+f_d\cdot \mathrm{n}\cdot T_r \right] +\mathrm{k}\cdot \varphi _A+\varphi _0
%         \\
%         &\mu =B/T_r, \tau _0=2R_0/c, f_d=2v/c, \varphi _A=\frac{2\pi}{\lambda}d\sin \theta ,
%         \\
%         &\mathrm{m}\in \left[ 0,N_f-1 \right] , \mathrm{n}\in \left[ 0,N_s-1 \right] , \mathrm{k}\in \left[ 0,N_a-1 \right] 
%     \end{aligned}
% \end{equation}
% where $N_f$, $N_s$, and $N_a$ are the number of sampling points, chirps, and virtual antennas, respectively. $B$ and $\lambda$  denote the bandwidth and wavelength of the FMCW waveform, while $T_s$ and $T_r$ denote the sampling period and chirp period. $d$ and $c$ are respectively the space distance of adjacent virtual antenna and light speed. 

\begin{figure}[h]
\centering
\includegraphics[width=1.0\columnwidth]{Figures/RadarData.pdf}
\caption{Radar data formats}
\label{data_vis}
\end{figure}
In automotive industry, multiple-input, multiple-output (MIMO) frequency-modulated continuous-wave (FMCW) radars are adopted \cite{zhou2022towards} to balance cost, size and performance. Each transmitting anttenas(Tx) transmit a sequence of FMCW waveforms, also named chirps, will be reflected by objects and returned to the receiving antennas(Rx). Then the echo signal will be first mixed with corresponding emitted signal and then passed through a low pass filter, so as to obtain the intermediate frequency (IF) signal. The discretely sampled IF signal, which includes the phase difference of emitted and returned signal, is called \textbf{ADC data}\cite{sun2020mimo}. 

Because of the continuous-wave nature, the IF signal of a chirp contains a frequency shift caused by the time delay of traveling between radar and objects. Then the radial distance of obstacles can be extracted by applying Fast Fourier Transform (FFT) on each chirp (range-FFT). The resulting complex signal is denoted as \textbf{range-time (RT) data}. Next, a second FFT along different chirps is conducted to extract the phase shift between two chirps caused by the motion of targets. The derived data is named \textbf{range-Doppler (RD) spectrum}. We denote $N_{Tx}$ and $N_{Rx}$ respectively as the number of transmit and receive antennas. And each grid on the RD spectrum has $N_{Tx}$ by $N_{Rx}$ channels. The small distance between adjacent virtual antennas leads to phase shift among different antennas, which is dependent on the AoA. Thus a third FFT (angle-FFT) can be applied along the channel axis to unwrap AoA. 
The AoA can be further decoded to azimuth and elevation based on the radar anttena calibration. The final real 3D tensor is referred to as the \textbf{range-azimuth-doppler (RAD) tensor}. 

If point cloud is desired, the RD spectrum will be first processed by CFAR algorithm to filter out peaks as candidate points. Then the angle-FFT will only be executed on these points. Final \textbf{radar point clouds (PCD)} consists of 3D coordinates, speed, and reflective intensity. In traditional radar signal processing, there is another data format named \textbf{range azimuth (RA) map}, which is obtained by decoding the azimuth of a single elevation on the RD spectrum and compressing the Doppler dimension to one channel. For comprehensive analyses, we include this modality in our experiments as well. The data formats mentioned above are illustrated in Figure \ref{data_vis}.
\section{Methods}
\label{headings}
\subsection{Overall Structure}
\begin{figure}[h]
\centering
\includegraphics[width=1.0\columnwidth]{Figures/Pipeline.pdf}
\caption{Overall pipeline of the proposed EchoFusion. H and W are height and weight of the image, while R, A, and T are the bin number of range, azimuth, and slow-time dimension, respectively.}
\label{pipeline}
\end{figure}

The overall architecture of our model is shown in Figure \ref{pipeline}.  First, we use separate backbones and FPNs \cite{lin2017feature} to extract multi-level features from RT radar maps and images. Then the polar queries aggregate camera features and radar features by deformable attention\footnote{cite sth}. Finally, the multi-scale polar BEV map will be passed through a transformer-based decoder. The final score and bounding box predictions can be obtained by decoding the output object queries. 

% \subsection{Radar Data Preprocessing}
% The range FFT results in a complex 3D tensor of shape ($B_R$, $B_S$, $N_{Rx}$), in which $B_R$, $B_S$, and $N_{Rx}$ are respectively numbers of discretization bins of range and slow-time dimension and the number of receiving antennas. Due to Doppler domain multiplexing (DDM), the same object will be visible $N_{Tx}$ times, one per emitting antenna \cite{rebut2022raw}.  In detail, on the RD spectrum, the object of range $R$ and relative radial velocity $D$ will appear at range-Doppler positions $\left[ \left( R, \left( D+n_{Tx}\varDelta \right) \mathrm{mod}\left( D_{\max} \right) \right) \right] _{n_{Tx}=1,..., N_{Tx}}$. $\varDelta$ is the Doppler shift generated by DDM, and $D_{\max}$ is the largest measurable Doppler values. 

% On the range-slow-time data, it is required to convert the phase shift in the Doppler domain to the slow-time domain. Based on the translation rule of DFT \cite{gonzalez2008digital}, the $n_{Tx}$-th transmitter corresponds to signal of 
% \begin{equation}
%     \hat{f}\left( b_R,b_S,n_{Rx},n_{Tx} \right) =f\left( b_R,b_S,n_{Rx} \right) \exp \left( -j2\pi \frac{n_{Tx}\varDelta \cdot b_S}{D_{\max}} \right) 
% \end{equation}
% where $f$ and $\hat{f}$ are respectively feature of input and output complex tensor. By applying this formulation and merging the last two channels, the signal intricacy will be solved, which facilitates further angle information extraction of the network. 

\subsection{Complementary Modality Fusion}
The core of our EchoFusion is how to fuse the camera and radar-slow-time data. We fuse them using a novel strategy named Polar Aligned Fusion (PAFusion). We start from multi-level features extracted by backbones and FPNs of radar and camera. Given the scale level of $l$, suppose that the corresponding image feature is in the shape of $H_l\times W_l\times C$. %where $H_l$, $W_l$, and $C$ are the height, width, and feature number of the feature map. 
And $\boldsymbol{f_{l,w}}\in \mathbb{R} ^{H_l\times C}$ denotes features  of tokens contained in $w$-th column. The initialized polar rays are in the shape of $R_l\times W_l\times C$, which has the same width and feature number, but different heights $R_l$ decided by the range span. Let $\boldsymbol{p_{l,w}}\in \mathbb{R} ^{R_l\times C}$ denote the polar ray of $w$-th column, then the azimuth-aligned cross attention can be formulated as follows:
\begin{equation}
    \begin{aligned}
        &\hat{\boldsymbol{p}}_{\boldsymbol{l},\boldsymbol{w}}=\mathrm{MultiHead}\left( \boldsymbol{p}_{\boldsymbol{l},\boldsymbol{w}},\bar{\boldsymbol{f}}_{\boldsymbol{l},\boldsymbol{w}},\bar{\boldsymbol{f}}_{\boldsymbol{l},\boldsymbol{w}} \right) =\mathrm{Concat}\left( \boldsymbol{z}^{\left( \boldsymbol{1} \right)},...,\boldsymbol{z}^{\left( \boldsymbol{n} \right)} \right) \boldsymbol{W}_{\boldsymbol{l}}^{\boldsymbol{O}}
        \\
        &\boldsymbol{z}^{\left( \boldsymbol{n} \right)}=\mathrm{Attention}\left( \boldsymbol{p}_{\boldsymbol{l},\boldsymbol{w}}\boldsymbol{W}_{\boldsymbol{l},\boldsymbol{n}}^{\boldsymbol{Q}},\bar{\boldsymbol{f}}_{\boldsymbol{l},\boldsymbol{w}}\boldsymbol{W}_{\boldsymbol{l},\boldsymbol{n}}^{\boldsymbol{K}},\bar{\boldsymbol{f}}_{\boldsymbol{l},\boldsymbol{w}}\boldsymbol{W}_{\boldsymbol{l},\boldsymbol{n}}^{\boldsymbol{V}} \right) 
    \end{aligned}
\end{equation}
where $\boldsymbol{\bar{f}_{l,w}}$ is the camera features with sine positional embedding. And $\boldsymbol{W}_{\boldsymbol{l},\boldsymbol{n}}^{\boldsymbol{Q}}\in \mathbb{R} ^{C\times C_{\mathrm{q}}}$, $\boldsymbol{W}_{\boldsymbol{l},\boldsymbol{n}}^{\boldsymbol{K}}\in \mathbb{R} ^{C\times C_{\mathrm{k}}}$, $\boldsymbol{W}_{\boldsymbol{l},\boldsymbol{n}}^{\boldsymbol{V}}\in \mathbb{R} ^{C\times C_{\mathrm{v}}}$, $\boldsymbol{W}_{\boldsymbol{l}}^{\boldsymbol{O}}\in \mathbb{R} ^{C\times C}$ are projection matrices. $C_{\mathrm{q}}=C_{\mathrm{k}}=C_{\mathrm{v}}=\mathrm{C}/n$, $n$ is the number of heads. 

The updated polar rays are stacked along the azimuth axis and form the polar feature map $\boldsymbol{\hat{P}_l}\in \mathbb{R} ^{R_l\times W_l\times C}$. In order to convert $\boldsymbol{\hat{P}_l}$ to a BEV feature map under radar coordinate system, a series of 3D points $S_{l}^{3D}=\left\{ \left( \rho _i,\phi _j,z_k \right) |i\in \left[ 1,R_l \right],j\in \left[ 1,A_l \right] ,k\in \left[ 1,Z_l \right] \right\} $ within the field of view (FoV) of the camera are generated. $A_l$ and $Z_l$ are respectively the number of points scattered in azimuth and z dimensions. Then the points are projected to the polar plane points $S_{l}^{P}=\left\{ \left( r_x,w_y \right) |x\in \left[ 1,R_l \right] ,j\in \left[ 1,W_l \right] \right\} $ using shared range index and the calibration matrix of the camera \cite{jiang2022polarformer}. After that, the features of projected points are endowed with corresponding 3D points. By aggregating features along z-axis, the final polar BEV feature map $\boldsymbol{G}_{\boldsymbol{l}}^{\boldsymbol{bev}}\in \mathbb{R} ^{R_l\times A_l\times C}$ can be obtained as follows:
\begin{equation}
    \begin{aligned}
        \boldsymbol{G_{l}^{bev}}\left( \rho _i,\phi _j \right) =\sum_{z=1}^{Z_l}{\lambda \left( \rho _i,\phi _j,z_k \right)}B\left( \boldsymbol{\hat{P}_l}, \left( r_x,w_y \right) \right) , \left( r_x,w_y \right) =\mathrm{Proj}\left( \rho _i,\phi _j,z_k|\boldsymbol{E},\boldsymbol{I},\boldsymbol{D} \right) 
    \end{aligned}
\end{equation}
where $\lambda$ is normalized weight, $B$ is the bilinear sampler, and $\mathrm{Proj}$ is the projection function utilizing extrinsic matrix $\boldsymbol{E}$, intrinsic matrix $\boldsymbol{I}$ and distortion coefficient $\boldsymbol{D}$. 

Let $\boldsymbol{D}_{\boldsymbol{l}}\in \mathbb{R} ^{R_l\times \varTheta _l\times C}$ denotes the radar BEV feature map of $l$-th level, where $\varTheta _l$ is the width. Since radar is already under the same polar coordinate system, the radar bin with the range index $\rho$ can directly interact with BEV bins with the same index. In particular, it can be formulated as follows:
\begin{equation}
    \begin{aligned}
        &\hat{\boldsymbol{g}}_{\boldsymbol{l},\boldsymbol{\rho }}=\mathrm{MultiHead}\left( \bar{\boldsymbol{g}}_{\boldsymbol{l},\boldsymbol{\rho }},\bar{\boldsymbol{d}}_{\boldsymbol{l},\boldsymbol{\rho }},\bar{\boldsymbol{d}}_{\boldsymbol{l},\boldsymbol{\rho }} \right) =\mathrm{Concat}\left( \boldsymbol{z'}^{\left( \boldsymbol{1} \right)},...,\boldsymbol{z'}^{\left( \boldsymbol{n} \right)} \right) \boldsymbol{W'}_{\boldsymbol{l}}^{\boldsymbol{O}}
        \\
        &\boldsymbol{z'}^{\left( \boldsymbol{n} \right)}=\mathrm{Attention}\left( \bar{\boldsymbol{g}}_{\boldsymbol{l},\boldsymbol{\rho }}\boldsymbol{W'}_{\boldsymbol{l},\boldsymbol{n}}^{\boldsymbol{Q}},\bar{\boldsymbol{d}}_{\boldsymbol{l},\boldsymbol{\rho }}\boldsymbol{W'}_{\boldsymbol{l},\boldsymbol{n}}^{\boldsymbol{K}},\bar{\boldsymbol{d}}_{\boldsymbol{l},\boldsymbol{\rho }}\boldsymbol{W'}_{\boldsymbol{l},\boldsymbol{n}}^{\boldsymbol{V}} \right)  
    \end{aligned}
\end{equation}
in which $\bar{\boldsymbol{g}}_{\boldsymbol{l},\boldsymbol{\rho }}\in \mathbb{R} ^{A_l\times C}
$ and $\bar{\boldsymbol{d}}_{\boldsymbol{l},\boldsymbol{\rho }}\in \mathbb{R} ^{\varTheta _l\times C}$ are respectively BEV feature and radar feature of tokens contained in $\rho$-th row. And $\boldsymbol{W'}_{\boldsymbol{l},\boldsymbol{n}}^{\boldsymbol{Q}}\in \mathbb{R} ^{C\times C_{\mathrm{q}}}$, $\boldsymbol{W'}_{\boldsymbol{l},\boldsymbol{n}}^{\boldsymbol{K}}\in \mathbb{R} ^{C\times C_{\mathrm{k}}}$, $\boldsymbol{W'}_{\boldsymbol{l},\boldsymbol{n}}^{\boldsymbol{V}}\in \mathbb{R} ^{C\times C_{\mathrm{v}}}$, $\boldsymbol{W'}_{\boldsymbol{l}}^{\boldsymbol{O}}\in \mathbb{R} ^{C\times C}$ are projection matrices. $C_{\mathrm{q}}=C_{\mathrm{k}}=C_{\mathrm{v}}=\mathrm{C}/n$, $n$ is the number of heads. After that, $\{\hat{\boldsymbol{g}}_{\boldsymbol{l},\boldsymbol{\rho }}|\rho=1,...,R_l\}$ are stacked along range dimension and form the final out put BEV feature map $\hat{\boldsymbol{G}}_{\boldsymbol{l}}\in \mathbb{R} ^{R_l\times A_l\times C}$.

By applying this cross-attention strategy, the fusion module is no longer bothered by the mismatched FoV between radar and camera. The row and column attention elaborately get around the problem of the image lacking a range dimension and the RT data of radar lacking an explicit azimuth dimension.
%, and alignment uncertainty caused by low-resolution sensing ability of specific direction. 
Besides, this structure can be easily extended to LiDAR or other data formats of radar, which facilitates exploring the effects of different modalities.

\subsection{Head and Loss}
We follow polar BEV decoders \cite{jiang2022polarformer} to decode multi-level BEV features and make predictions from object queries. Since velocity prediction is not included in our tasks, we delete the corresponding branches. The regression targets include ($d_\rho$, $d_\phi$, $d_z$, $\mathrm{log}\space l$, $\mathrm{log}\space w$, $\mathrm{log}\space h$, $\mathrm{sin}(\theta_{ori}-\phi)$, $\mathrm{cos}(\theta_{ori}-\phi)$), where $d_\rho$, $d_\phi$, $d_z$ are relative offset to the reference point ($\rho$, $\phi$, $z$), $l$, $w$, $h$, $\theta_{ori}$ are length, width,  height, and orientation of bounding box. The classification and regression tasks are respectively supervised by Focal loss \cite{lin2017focal} and F1 loss.

==> Sections/3_method_v2.tex <==
\section{Preliminary}
\label{preliminary}
% If an object with radial speed $v$ has a radial distance $R_0$ and angle of arrival (AoA) $\theta$ to the radar, it will have a complex response on ADC data with phase:
% \begin{equation}
%     \label{phase}
%     \begin{aligned}
%         &P_{D}^{H}\left( \mathrm{m},\mathrm{n},\mathrm{k} \right) \approx 2\pi \left[ -\mu \cdot \tau _0\cdot \mathrm{m}\cdot T_s+f_d\cdot \mathrm{n}\cdot T_r \right] +\mathrm{k}\cdot \varphi _A+\varphi _0
%         \\
%         &\mu =B/T_r, \tau _0=2R_0/c, f_d=2v/c, \varphi _A=\frac{2\pi}{\lambda}d\sin \theta ,
%         \\
%         &\mathrm{m}\in \left[ 0,N_f-1 \right] , \mathrm{n}\in \left[ 0,N_s-1 \right] , \mathrm{k}\in \left[ 0,N_a-1 \right] 
%     \end{aligned}
% \end{equation}
% where $N_f$, $N_s$, and $N_a$ are the number of sampling points, chirps, and virtual antennas, respectively. $B$ and $\lambda$  denote the bandwidth and wavelength of the FMCW waveform, while $T_s$ and $T_r$ denote the sampling period and chirp period. $d$ and $c$ are respectively the space distance of adjacent virtual antenna and light speed. 

\begin{figure}[t]
\centering
\includegraphics[width=1.0\columnwidth]{Figures/RadarData.pdf}
\caption{Radar data formats used in this paper. All the axes that have physical meanings are labeled with units. Due to Doppler domain multiplexing (DDM), the real speed is periodic on the Doppler dimension, which is hard to label. We use the index number of the Doppler dimension instead. }
\label{data_vis}
\end{figure}

In the automotive industry, multiple-input, multiple-output (MIMO) frequency-modulated continuous-wave (FMCW) radars are adopted \cite{zhou2022towards} to balance cost, size, and performance. Each transmitting antenna (Tx) transmits a sequence of FMCW waveforms, also named chirps, which will be reflected by objects and returned to the receiving antennas (Rx). Then the echo signal will be first mixed with the corresponding emitted signal and then passed through a low pass filter, so as to obtain the intermediate frequency (IF) signal. The discretely sampled IF signal, which includes the phase difference of emitted and returned signal, is called \textbf{ADC data}\cite{sun2020mimo}. The ADC data has three dimensions, fast time, slow time, and channel, which have physical correspondence with range, speed, and angle respectively.

Because of the continuous-wave nature, the IF signal of a chirp contains a frequency shift caused by the time delay of traveling between radar and objects. Then the radial distance of obstacles can be extracted by applying Fast Fourier Transform (FFT) on each chirp, i.e. fast-time dimension. This FFT operation is also called range-FFT. The resulting complex signal is denoted as \textbf{range-time (RT) data}. Next, a second FFT (Doppler FFT) along different chirps, i.e. slow-time dimension, is conducted to extract the phase shift between two chirps caused by the motion of targets. The derived data is named \textbf{range-Doppler (RD) spectrum}. We denote $N_{Tx}$ and $N_{Rx}$ respectively as the number of transmitting and receiving antennas. And each grid on the RD spectrum has $N_{Tx} \times N_{Rx}$ channels. The small distance between adjacent virtual antennas leads to phase shifts among different antennas, which is dependent on the AoA. Thus a third FFT (angle-FFT) can be applied along the channel axis to unwrap AoA. 
The AoA can be further decoded to azimuth and elevation based on the radar antenna calibration. The final 4D tensor is referred to as the \textbf{range-elevation-azimuth-Doppler (READ) tensor}. 

If a point cloud is desired, the RD spectrum will be first processed by the CFAR algorithm to filter out peaks as candidate points. Then the angle-FFT will only be executed on these points. Final \textbf{radar point cloud (PCD)} consists of 3D coordinates, speed, and reflective intensity. In traditional radar signal processing, there is another data format named \textbf{range-azimuth (RA) map}, which is obtained by decoding the azimuth of a single elevation on the RD spectrum and compressing the Doppler dimension to one channel. For comprehensive analyses, we include this modality in our experiments as well. The data formats mentioned above are illustrated in Figure \ref{data_vis}, except for READ tensor because it is difficult to visualize.
\section{Methods}

In this section, we will introduce our network design. Firstly we will give a brief introduction of the whole pipeline in Section \ref{overall_structure}. Then our proposed Polar-Aligned Attention module will be detailedly described in Section \ref{Column-wise Image Fusion}. Finally, the detection head and loss functions are introduced in Section \ref{head_loss}.

\label{headings}
\subsection{Overall Structure}
\label{overall_structure}
\begin{figure}[t]
\centering
\includegraphics[width=1.0\columnwidth]{Figures/Pipeline.pdf}
\caption{Overall pipeline of the proposed EchoFusion. H and W are the height and weight of the image, while R, A, and T are the bin number of range, azimuth, and Doppler dimension, respectively. The \textcolor[rgb]{1,0,0}{Coord. Mapping} in the figure is explained in section \ref{Column-wise Image Fusion}.}
\label{pipeline}
\end{figure}

The overall architecture of our model is shown in Figure \ref{pipeline}.  First, we use separate backbones and FPNs \cite{lin2017feature} to extract multi-level features from RT radar maps and images. Then the polar queries aggregate camera features and radar features by cross-attention. Finally, the multi-scale polar BEV map will be passed through a transformer-based decoder with object queries. The final score and bounding box predictions can be obtained by decoding the output object queries. The core of our EchoFusion is how to fuse the camera and radar slow-time data. We fuse them using a novel strategy named Polar Aligned Attention (PA-Attention). In the next two subsections, we will explain this strategy in detail.

% \subsection{Radar Data Preprocessing}
% The range FFT results in a complex 3D tensor of shape ($B_R$, $B_S$, $N_{Rx}$), in which $B_R$, $B_S$, and $N_{Rx}$ are respectively numbers of discretization bins of range and slow-time dimension and the number of receiving antennas. Due to Doppler domain multiplexing (DDM), the same object will be visible $N_{Tx}$ times, one per emitting antenna \cite{rebut2022raw}.  In detail, on the RD spectrum, the object of range $R$ and relative radial velocity $D$ will appear at range-Doppler positions $\left[ \left( R, \left( D+n_{Tx}\varDelta \right) \mathrm{mod}\left( D_{\max} \right) \right) \right] _{n_{Tx}=1,..., N_{Tx}}$. $\varDelta$ is the Doppler shift generated by DDM, and $D_{\max}$ is the largest measurable Doppler values. 

% On the range-slow-time data, it is required to convert the phase shift in the Doppler domain to the slow-time domain. Based on the translation rule of DFT \cite{gonzalez2008digital}, the $n_{Tx}$-th transmitter corresponds to signal of 
% \begin{equation}
%     \hat{f}\left( b_R,b_S,n_{Rx},n_{Tx} \right) =f\left( b_R,b_S,n_{Rx} \right) \exp \left( -j2\pi \frac{n_{Tx}\varDelta \cdot b_S}{D_{\max}} \right) 
% \end{equation}
% where $f$ and $\hat{f}$ are respectively feature of input and output complex tensor. By applying this formulation and merging the last two channels, the signal intricacy will be solved, which facilitates further angle information extraction of the network. 

\subsection{Column-wise Image Fusion}
\label{Column-wise Image Fusion}
After obtaining image and radar features from corresponding encoders, we first initialize the $l$-th level polar queries $\boldsymbol{Q}_{\boldsymbol{l}}\in \mathbb{R} ^{R_l\times A_l\times d}$ uniformly in polar BEV space. Here, $R_l$, $A_l$, and $d$ respectively denote the shape of range, azimuth, and channel dimensions. For brevity, we omit $l$ in the following two subsections. Given a query $q\in \mathbb{R} ^d$ located at $(r_{bev}, \phi_{bev})$, it corresponds to a pillar centered at $(r_{bev}, \phi_{bev})$ with infinite height. Taking the coordinate system defined in RADIal \cite{rebut2022raw}, $x_R$, $y_R$, and $z_R$ axes respectively points to the right, front, and upright, while subscript $R$ means radar coordinate. Similarly, the camera coordinates are denoted as $(x_C, y_C, z_C)$, which points to the right, up, and back, respectively. Thus we have correspondence as follows:
\begin{equation}
    \label{w-polar}
    x_R=r_{bev}\cos \left( \phi _{bev} \right), \quad y_R=r_{bev}\sin \left( \phi _{bev} \right).
\end{equation}
Using extrinsic matrix and intrinsic matrix, we have the following formulation:
\begin{equation}
    \label{in-ex}
    \frac{x_I-u_0}{f_x}=\frac{x_C}{z_C},  \quad \left( \begin{array}{c}
	x_C\\
	y_C\\
	z_C\\
    \end{array} \right) =R \left( \begin{array}{c}
    	x_R\\
    	y_R\\
    	z_R\\
        1\\
    \end{array} \right) + T, 
\end{equation}
where $u_0$, $f_x$ are principal point offset and focal length on $x$-axis in the intrinsic matrix, $x_I$ is the image column index that corresponds to the point $(x_R, y_R, z_R)$, while $R$ and $T$ are rotation matrix and translation vector of the calibration matrix between camera and radar, respectively. Under mild conditions, we can derive that the pillar exactly matches a specific column in the image. Limited by the number of pages, we leave detailed proof in the appendix.
% In the standard sensor setting of ADS, the front camera, LiDAR, and radar are  parallel to roads, pointing in the driving direction. This enables the rotation matrix to only involve a 90-degree rotation around the right x-axis of the radar coordinate, i.e. $|\alpha |=\pi /2$, $\beta =\gamma =0$, where $\alpha$, $\beta$, $\gamma$ are respectively Euler angles roll, pitch, and yaw correlated with rotation matrix R. And it is also the exact case in the RADIal dataset. With this precondition and assuming that $\alpha=\pi /2$, we re-express the $x_I$ using $r_{bev}$ and $\phi_{bev}$ as follows:
% \begin{equation}
%     \label{r_phi_to_x}
%     x_I=u_0+f_x\frac{r_{bev}\cos \left( \phi _{bev} \right) + t_x}{r_{bev}\sin \left( \phi _{bev} \right) +  t_z},
% \end{equation}
% which means the pillar exactly matches a specific column in the image.

However, the $z_R$ coordinate is not specified for a query, while for a pixel $(x_I, y_I)$ on the monocular image, its depth is unknown as well. Thus we cannot precisely corresponds a query to the image feature, while we can correspond queries of the same azimuth to the same column of images. Enlightened by this observation, we use a versatile cross-attention mechanism to flexibly aggregate required features from images. %In detail, we can first collect features of all the locations in the column corresponding with the pillar. 
Namely, all the queries with the same azimuth form the query matrix, while all the features in the corresponding column in the image form the key and value matrix.
%Consequently, the cross-attention \cite{vaswani2017attention} is utilized to update query $q$. 
Formally, these two steps can be expressed as follows:
\begin{equation}
    \begin{aligned}
        F_I( x_I, \cdot) &=\mathrm{Stack}\left( [ f_I\left( x_I,y_I \right)] \right) \in \mathbb{R} ^{H_l\times d}, \quad \forall y_I \in [0,H_l-1], \\
        \hat{q}\left( r_{bev},\phi _{bev} \right) &=\mathrm{CrossAttn}\left( q\left( r_{bev},\phi _{bev} \right) , F_I\left( x_I,\cdot \right) , F_I\left( x_I,\cdot \right) \right) ,
    \end{aligned}
\end{equation}
where $f_I( x_I,y_I)$ is the image feature located at $x_I,y_I$.

\subsection{Range-wise Radar Fusion}
\label{Range-wise Radar Fusion}
We denote updated BEV queries as $\hat{\boldsymbol{Q}}_{\boldsymbol{l}}\in \mathbb{R} ^{R_l\times A_l\times d}
$. After that, it will be used to sample features from radar. Since the radar feature map shares the same space partition with the BEV queries, the updated query $\hat{q}\left( r_{bev},\phi _{bev} \right)$ exactly matches the same range index of the radar feature, i.e. $r_R=r_{bev}$.
To aggregate all the features from all chirps in one frame, we perform cross attention for a certain query $\hat{q}$ with the row $r_R$ in RT map as key and value. Formally,
%However, the slow-time correspondence of $\hat{q}\left(r_{bev},\phi _{bev} \right)$ is non-trivial to determine because this dimension doesn't exist in the polar BEV query. But using a similar strategy, we can bypass this problem. With radar row index $r_R$, we can collect all the radar bins located in this row as keys and values. The cross-attention \cite{vaswani2017attention} is then applied to update query $\hat{q}$. These two steps can be formulated as follows:
\begin{equation}
    \begin{aligned}
        G_R( r_R, \cdot ) &=\mathrm{Stack}\left( [ g_R( r_R,t_R )] \right) \in \mathbb{R} ^{R_l\times d}, \quad \forall t_R \in [0,T_l-1] ,
        \\
        \tilde{q}\left( r_{bev},\phi _{bev} \right) &=\mathrm{CrossAttn}\left( \hat{q}\left( r_{bev},\phi _{bev} \right) , G_R\left( r_R, \cdot \right) , G_R\left( r_R, \cdot \right) \right) ,
        %\\
        %&=\mathrm{CrossAttn}\left( \hat{q}\left( r_{bev},\phi _{bev} \right) ,G_R\left( r_{bev} \right) , G_R\left( r_{bev} \right) \right) 
    \end{aligned}
\end{equation}
where $R_l$ and $T_l$ are the height and width of the radar feature map, and  $g_R\left( r_R,t_R \right) \in \mathbb{R} ^d$ is the radar feature of position $(r_R, t_R)$.

%For the radar echoes belonging to a specific range, their azimuth distribution can be fully described by all bins scattered in the corresponding row. And thus the query can inherently learn how to capture the required information to help locate the correct position of objects.

%By applying this cross-attention strategy, the fusion module is no longer bothered by the mismatched FoV between radar and camera. The row and column attention elaborately get around the problem of the image lacking a range dimension and the RT data of radar lacking an explicit azimuth dimension.
%, and alignment uncertainty caused by low-resolution sensing ability of specific direction. 
%Besides, this structure can be easily extended to LiDAR or other data formats of radar, which facilitates exploring the effects of different modalities.

Note that though we don't explicitly decode AoA as in RA map, the AoA has been implicitly encoded in the phase difference of the response of different virtual antenna. Consequently, it can be learned from the features in RT map indirectly.

%We also try to use RA map in ablation study. Although it is also in polar coordinate, the azimuth resolution is different from that of the BEV queries. For implementation simplicity, we still conduct the same attention mechanism as RT.

\subsection{Head and Loss}
\label{head_loss}
We follow polar BEV decoders \cite{jiang2022polarformer} to decode multi-level BEV features and make predictions from object queries. Since we don't have velocity annotation on this dataset, we remove the corresponding branch. The regression targets include ($d_\rho$, $d_\phi$, $d_z$, $\mathrm{log}\space l$, $\mathrm{log}\space w$, $\mathrm{log}\space h$, $\mathrm{sin}(\theta_{ori}-\phi)$, $\mathrm{cos}(\theta_{ori}-\phi)$), where $d_\rho$, $d_\phi$, $d_z$ are relative offset to the reference point ($\rho$, $\phi$, $z$), $l$, $w$, $h$, $\theta_{ori}$ are length, width,  height, and orientation of bounding box. The classification and regression tasks are respectively supervised by Focal loss \cite{lin2017focal} and L1 loss.

==> Sections/4_experiments.tex <==
\section{Experiments}
In this section, we conduct thorough experiments to validate the effectiveness of our approach. We first introduce the dataset and metrics used in our experiments, then followed by comparisons with other state-of-the-art methods. Lastly, we ablate some designs and potential input format of raw radar data in our method, and discuss some limitations.
\label{exp}
\subsection{Experimental Settings}
\textbf{The RADIal Dataset} \cite{rebut2022raw} provides 8252 annotated frames with synchronized multi-sensor data. Training, validation, and test sets contain 6231, 986, and 1035 frames, respectively. Each object is annotated with a 3D center coordinate of the visible face of the vehicle. The size and orientation of the objects are pre-defined templates, i.e. they are the same for all objects. In the evaluation, precisions and recalls under ten thresholds are calculated, The average precision (AP), average recall (AR), and F1 score are obtained through the ten precisions and ten recalls as the evaluation metric. Range error (RE) and azimuth error (AE) are also reported to evaluate localization accuracy. The annotation method and metrics are quite different with common autonomous driving datasets \cite{caesar2020nuscenes,sun2020scalability}. Nonetheless, to compare with state-of-the-art methods, we still list our results using the metrics defined in RADIal \cite{rebut2022raw} as a reference.

\textbf{Re-annotation and more metrics.} Based on the provided LiDAR point cloud, we have refined the annotation to 3D bounding box form, which includes center position, scale, and heading in 3D space. Capitalizing on these new annotations, we are able to apply metrics that are vastly used in 3D object detection tasks. Specifically, we take AP defined in Waymo dataset \cite{sun2020scalability} as our main metrics. Since the LiDAR used in RADIal is only 16-beam, we cannot label accurate height for the objects. So we mainly utilize BEV IoU for evaluation. We use the threshold of 0.7 for normal IoU and longitudinal error-tolerant (LET) IoU computation\cite{hung2022let}. 
%Under 3D evaluation, we take 0.5 as the IoU threshold due to relatively low vertical annotation accuracy. 
Considering the spatial distribution of ground-truth, the distance evaluation is further broken down into
two categories: 0 to 50 meters, 50 to 100 meters. For a more comprehensive evaluation, we also introduce the error metrics defined in nuScenes dataset\cite{caesar2020nuscenes}, including  ATE, ASE, and AOE for measuring errors of translation, scale, and orientation. 

\textbf{Radar Formats.} As introduced in Section \ref{preliminary}, there are multiple formats of radar raw data, such as ADC, RT, RD, READ. These formats can be converted sequentially by FFT, which is a linear operation that can be absorbed into the linear layers. So from the perspective of neural network, these formats are equivalent. However, our proposed Polar-Aligned Attention requires a range dimension for indexing key and value in cross-attention, so we choose RT as a representative in the experiments. We also conduct experiments on RA to investigate the necessity of explicit azimuth.

\textbf{Implementation Details.} All our experiments are carried out on eight 3090 GPUs with the same batch size of 8. For the image backbone, we adopt ResNet-50 with pre-trained weights provided by BEVFormer \cite{li2022bevformer}. For LiDAR and radar point cloud branch, we borrow the voxel encoder from PointPillar \cite{lang2019pointpillars} and use ResNet-50 with modified strides as the backbone. Other representations of radar share similar modified ResNet-50 as the backbone, but with an extra 1 $\times$ 1 convolution at the beginning for channel number alignment. It is worth noticing that the RT map needs to be pre-processed to decode the echo of each virtual antenna\cite{rebut2022raw}. To prevent overfitting, the image-only variant is trained for only 12 epochs while others are trained for 24 epochs. AdamW \cite{loshchilov2017decoupled} is adopted as the optimizer and a learning rate of 5e-5 is shared for all models. 
Due to the limited size of the dataset, we find that the results are unstable across different runs. To make a fair comparison, each experiment is repeated three times. In modality ablation, we show the mean and variance of each experiment result.

\subsection{Comparison to State-of-the-art Methods}
\begin{table}
  \caption{Point-based detection performances on RADIal Dataset test split. C, RD, and RT respectively refer to camera, radar-Doppler spectrum, and radar-time data. Our method achieves the best performance in both average precision (AP), average recall (AR), and F1-score (F1). The best result of each metric is in \textbf{bold}.}
  \label{sota}
  \centering
  \resizebox{0.85\textwidth}{!}{%
  \begin{tabular}{lllllll}
    \toprule
    Methods & Modality & AP($\%$)$\uparrow$ & AR($\%$)$\uparrow$ & F1($\%$)$\uparrow$ & RE(m)$\downarrow$ & AE($^{\circ}$)$\downarrow$ \\
    \midrule
    FFTRadNet \cite{madani2022radatron} & RD & 96.84 & 82.18 & 88.91 & \textbf{0.11} & 0.17 \\
    T-FFTRadNet \cite{giroux2023t} & ADC & 89.60 & 89.50 & 89.50 & 0.15 & 0.12 \\
    ADCNet \cite{yang2023adcnet} & ADC & 95.00 & 89.00 & 91.90 & 0.13 & \textbf{0.11} \\
    CMS \cite{jin2023cross} & RD\&C & 96.90 & 83.50 & 89.70 & 0.45 & n/a \\
    EchoFusion & RT\&C & \textbf{96.95} & \textbf{93.43} & \textbf{95.16} &0.12 & 0.18 \\
    \bottomrule
  \end{tabular}
  }
\end{table}

We first compare our method with state-of-the-art detectors on AP, AR, range error, and azimuth error defined in RADIal \cite{rebut2022raw}, with original object-level point annotations\footnote{The official implementation of these metrics are different from common implementations. Specifically, AP and AR are averaged on score thresholds from 0.1 to 0.9 with step of 0.1 and IoU threshold of 0.5. And F1 score is directly calculated from AP and AR defined above.}. The results are illustrated in Table \ref{sota}. Our method significantly improves AR and F1 performance and achieves a remarkable improvement over all existing detectors including CMS \cite{jin2023cross} which also integrates both radar raw data and camera data. Note that RE and AE are not quite informative because these two metrics are calculated on all the recalled objects of a method, which is unfair to high-recall models like ours.

\begin{table}
  \caption{BEV detection performances on RADIal Dataset test split with refined 3D ground-truth bounding box. C, RD, and RT respectively refer to camera, range-Doppler spectrum, and range-time data. The best result of each metric is in bold. Our method exceeds FFTRadNet by a large margin.}
  \label{sota_newlabel}
  \centering
  \resizebox{0.99\textwidth}{!}{%
  \begin{tabular}{llllllll}
    \toprule
    & & \multicolumn{3}{c}{BEV AP@0.7($\%$)$\uparrow$}&\multicolumn{3}{c}{LET-BEV-AP@0.7($\%$)$\uparrow$}\\
    \cmidrule(r){3-5} \cmidrule(r){6-8}
     Methods & Modality & Overall & 0 - 50m & 50 - 100m & Overall & 0 - 50m & 50 - 100m \\
    \midrule
    FFTRadNet3D\cite{rebut2022raw} & RD & 57.26 & 68.66 & 52.28 & 62.81 & 75.55 & 57.98 \\
    EchoFusion & RT\&C & \textbf{84.25} & \textbf{86.67} & \textbf{90.48} & \textbf{88.54} & \textbf{92.10} & \textbf{94.45} \\
    \bottomrule
  \end{tabular}
  }
\end{table}

To evaluate in a more rigorous and informative way, we also conduct experiments on the refined annotations and vastly adopted metrics in 3D object detection. FFTRadNet\cite{rebut2022raw} is lifted up with additional branches to predict the scale and orientation of targets. We can only compare with this FFTRadNet variant since codes of other algorithms\cite{giroux2023t, jin2023cross, yang2023adcnet} are not available yet. The results in Table \ref{sota_newlabel} show that the proposed method outperforms FFTRadNet by a large margin. This significant improvement reveals the huge benefit of unleashing the power of radar data in multi-modality fusion.

\subsection{Ablation Study}
\begin{table}[!tb]
  \caption{Ablation studies on our EchoFusion. Complex means interpreting input features as real and imaginary (IQ) or magnitude and phase (MP). Pretrain means whether to use the pre-trained image backbone. The best result of each metric is in \textbf{bold}.}
  \label{arch}
  \centering
  \resizebox{0.9\textwidth}{!}{%
  \begin{tabular}{lllllllll}
    \toprule
    \multicolumn{2}{c}{Conditions} & \multicolumn{3}{c}{BEV AP@0.7($\%$)$\uparrow$}&\multicolumn{3}{c}{LET-BEV-AP@0.7($\%$)$\uparrow$}\\
    \cmidrule(r){1-2} \cmidrule(r){3-5} \cmidrule(r){6-8}
    Complex & Pretrain & Overall & 0 - 50m & 50 - 100m & Overall & 0 - 50m & 50 - 100m \\
    \midrule
    MP & w & \textbf{84.25} & 86.67 & \textbf{90.48} & \textbf{88.54} & 92.10 & \textbf{94.45} \\
    IQ & w & 82.64 & \textbf{87.09} & 87.81 & 88.06 & \textbf{92.25} & 93.24 \\
    MP & w/o & 74.34 & 81.26 & 78.71 & 78.90 & 85.44 & 84.28 \\
    \bottomrule
  \end{tabular}
  }
\end{table}

We ablate the input format to the radar feature extraction network in Table \ref{arch}. It shows that the interpretation of complex input can improve overall detection performance, especially for long-range perception. The magnitude and phase representation encodes a non-linear transformation of the complex representation, which may relate to the final prediction target better. We also tried to remove the pre-training of the image branch. The results drop significantly, which confirms that in this relatively small dataset, a good pre-training is crucial for good performance.

\subsection{Comparison of Different Modalities}
\begin{table}
  \caption{BEV detection performances of different modality combinations of our algorithm on RADIal Dataset test split. Refined 3D bounding box annotations are applied. C, L, RD, RT, RA, RP respectively refer to the camera, LiDAR, range-Doppler spectrum, range-time data, range-azimuth map, and radar point cloud. The best result without LiDAR of each metric are in \textbf{bold}, and the results with LiDAR are on gray background.}
  \label{modalities}
  \centering
  \resizebox{0.99\textwidth}{!}{%
  \begin{tabular}{lllllllllll}
    \toprule
    \multicolumn{5}{c}{Modality} & \multicolumn{3}{c}{BEV AP@0.7($\%$)$\uparrow$}&\multicolumn{3}{c}{LET-BEV-AP@0.7($\%$)$\uparrow$}\\
    \cmidrule(r){1-5} \cmidrule(r){6-8} \cmidrule(r){9-11}
    C & RT & RA & RP & L & Overall & 0 - 50m & 50 - 100m & Overall & 0 - 50m & 50 - 100m \\
    \midrule
    \checkmark & & & & & 10.85$\pm$0.01 & 23.84$\pm$0.68 & 1.83$\pm$0.29 & 54.31$\pm$1.58 & \textbf{78.67$\pm$1.64} & 32.10$\pm$0.37 \\
    & \checkmark & & & & 48.37$\pm$1.11 & 64.02$\pm$3.93 & 44.36$\pm$0.12 & 54.96$\pm$1.53 & 69.78$\pm$4.58 & 51.01$\pm$0.07 \\
    & & \checkmark & & & 51.19$\pm$0.88 & \textbf{65.83$\pm$1.41} & 43.31$\pm$0.28 & 58.49$\pm$0.15 & 73.48$\pm$0.27 & 51.16$\pm$0.52 \\
    & & & \checkmark & & \textbf{53.33$\pm$0.76} & 65.55$\pm$1.78 & \textbf{47.07$\pm$1.16} & \textbf{62.94$\pm$1.25} & 76.71$\pm$2.48 & \textbf{56.60$\pm$1.62} \\ \rowcolor{gray!20}
    & & & & \checkmark & 84.56$\pm$0.09 & 87.34$\pm$0.09 & 91.85$\pm$0.12 & 86.23$\pm$0.47 & 88.52$\pm$0.97 & 93.11$\pm$0.06 \\
    \midrule
    \checkmark & \checkmark & & & & 84.25$\pm$0.33 & 86.67$\pm$1.17 & 90.48$\pm$1.04 & 88.54$\pm$0.52 & 92.10$\pm$1.15 & 94.45$\pm$0.17 \\
    \checkmark & & \checkmark & & & \textbf{84.85$\pm$0.78}& \textbf{87.88$\pm$0.73} & \textbf{91.64$\pm$0.20} & \textbf{89.70$\pm$0.60} & \textbf{93.86$\pm$0.69} & \textbf{95.28$\pm$0.05} \\
    \checkmark & & & \checkmark & & 82.00$\pm$0.97 & 86.58$\pm$1.04 & 86.17$\pm$0.83 & 87.97$\pm$0.69 & 92.75$\pm$0.81 & 92.39$\pm$0.53 \\ \rowcolor{gray!20}
    \checkmark & & & & \checkmark & 87.05$\pm$0.71 & 88.88$\pm$1.71 & 95.43$\pm$0.23 & 88.97$\pm$0.27 & 91.55$\pm$1.64 & 96.15$\pm$0.59 \\ 
    %\rowcolor{gray!20}
    %\checkmark & & & \checkmark & \checkmark & 86.53$\pm$0.05 & 87.98$\pm$1.11 & 95.08$\pm$0.47 & 88.35$\pm$0.24 & 91.30$\pm$0.42 & 96.19$\pm$0.58 \\
    \bottomrule
  \end{tabular}
  }
\end{table}
To further study the effects of different modalities, we change the input format indicated in Figure \ref{data_vis} and corresponding backbones, and test with and without image modality. Table \ref{modalities} presents the results, and our findings are listed as follows.

\textbf{Comparing single-modality results} It is not surprising that LiDAR ranks first while the camera is the worst in terms of AP. Though poor in depth estimation, the camera has excellent angular resolution, which is beneficial for LET-BEV-AP. It achieves comparable results with radar in LET-BEV-AP. Besides, without the guidance of image, the radar-only network gets better performance as more hand-crafted post-processing is involved. However, their metrics still lag far from LiDAR.

\textbf{Comparing multi-modality with single modality} The power of radar data is released by fusing with image. No matter in what data format, all the radar raw representations gain around 30 points improvement by fusing with images. By combining image and range-time data, we obtain BEV AP that is only 0.03 less than that of LiDAR only method. And the LET-BEV-AP and long-range detection ability are even better. We argue that it is mainly because images provide enough clues to decode the essential information from raw radar representation.

\textbf{Comparing multi-modality results} When integrating with images, the LiDAR-fused method still outperforms other radar-fused methods. In terms of different representations of radar, both RT and RA outperform traditional cloud points, especially in the 50-100m range, in which the difference is as large as 4 points in AP. We owe this finding to the information loss and false alarm of radar point cloud as shown in Figure \ref{pcd}. The performance gap between RT and RA with camera modality is within the error bar, indicating that it is not necessary to explicitly solve the azimuth, nor necessary to permute the Doppler-angle dimensions as FFTRadNet\cite{rebut2022raw} does.
%On the other hand, the speed, azimuth, elevation, and range information in RT and RA data is never impaired by the hand-crafted radar data processing pipeline, which offers the best overall performance.


\subsection{Discussion and Limitations}
\label{subsec:discussion}
\begin{table}
  \caption{3D detection performances on RADIal Dataset test split with refined 3D ground-truth bounding box. C, L, and RT respectively refer to camera, LiDAR, and radar-time data. The best result of each metric is in bold.}
  \label{3DmAP}
  \centering
  \resizebox{0.75\textwidth}{!}{%
  \begin{tabular}{lllllll}
    \toprule
    & \multicolumn{3}{c}{3D AP@0.5($\%$)$\uparrow$}&\multicolumn{3}{c}{Average Error@0.5$\downarrow$}\\
    \cmidrule(r){2-4} \cmidrule(r){5-7}
     Modality & Overall & 0 - 50m & 50 - 100m & ATE & ASE & AOE\\
    \midrule
    L & 62.69 & 80.04 & 54.26 & 0.243 & \textbf{0.171} & 0.027 \\
    L\&C & \textbf{68.36} & \textbf{84.74} & \textbf{61.54} & \textbf{0.239} & 0.180 & \textbf{0.020} \\
    RT\&C & 39.81 & 56.05 & 31.24 & 0.301 & 0.173 & \textbf{0.020} \\
    \bottomrule
  \end{tabular}
  }
\end{table}
Firstly, it is worth noticing that although the overall performance of radar is improved by fusing with the camera, the performance in the short-range is lower than that in the long-range. We speculate the main reason is inaccurate annotation. The 16-beam LiDAR provided in RADIal is too sparse at a farther distance for annotators to give an accurate size for the long-range objects. In such cases, they are required to assign a template with a fixed size to these objects. These annotations make the problem much easier for farther distances, which leads to higher performance than near distances.
%However, this is not detrimental for neural networks, as predicting a fixed value is relatively straightforward for the networks.  
%the objects of large yaw are not common in the training set, and the predictions are not perfect. But in the test split, most of the objects with large rotations are concentrated in short range, thus harming the performance. 

Secondly, though the radial speed label is included in the original annotations of RADIal, radial speed is not quite useful for downstream modules like planning since they need accurate longitudinal and lateral velocity to predict whether the vehicles will interfere with the ego vehicle. However, the synchronized frames are not consecutive in this dataset, it is hard to label velocities for the objects. Considering these factors, velocity prediction is not included in our task. 

Finally, as shown in Table \ref{3DmAP}, our method still lags far from the LiDAR-only structure on 3D metrics. The reasons are two-fold. The 16-beam LiDAR 
still has considerable errors in the z-axis. From 30 meters on, the error has exceeded 0.3 meters, which makes accurate annotation infeasible. The elevation resolution of the radar is inferior to that of LiDAR, making it less favorable. As a result, the detector struggles to regress inaccurate elevation with more inaccurate measurements. This phenomenon can be alleviated by better radar antenna design.

==> Sections/6_supp_v2.tex <==

\setcounter{equation}{0}
\setcounter{table}{0}
\setcounter{figure}{0}
\setcounter{section}{0}
\renewcommand\theequation{S\arabic{equation}}
\renewcommand\thefigure{S\arabic{figure}}
\renewcommand\thetable{S\arabic{table}}
\renewcommand\thesection{\Alph{section}}

%In this supplementary material, we begin by providing detailed proof for section \ref{Column-wise Image Fusion} in \cref{sec:proof}, offering a detailed explanation of our methodology. Moving on to \cref{sec:data}, we present the visualization of detected results as well as the distribution of the RADIal dataset and elaborate on the rationale behind our range division. In Section \ref{sec:R&C}, we present additional experimental results that highlight the complementary nature of radar and camera modalities, providing further evidence of their synergistic effects. In \cref{sec:detail}, we offered BEV detection results when the radar-Doppler spectrum is taken as input radar format. Besides, the averaged 3D performances are also presented for a better understanding of our approach.

\section*{Supplementary Material}
\section{Proof for column and pillar correspondence}
\label{sec:proof}
In this section, we will provide a detailed proof for the correspondence between pillar in radar coordinate and column in camera coordinate as described in Section 4.2 of our main paper.

Suppose that the rotation matrix and translation vector between radar and camera are:
\begin{equation}
    R=\left( \begin{matrix}
	a_1&		b_1&		c_1\\
	a_2&		b_2&		c_2\\
	a_3&		b_3&		c_3\\
    \end{matrix} \right) , T=\left( \begin{array}{c}
    	d_1\\
    	d_2\\
    	d_3\\
    \end{array} \right). 
\end{equation}
Then for a point located at $(r_{bev}, \phi_{bev}, z)$ under radar's polar coordinate, it has cartesian coordinate $(x_R, y_R, z_R)$:
\begin{equation}
    x_R=r_{bev}\cos \left( \phi _{bev} \right) , y_R=r_{bev}\sin \left( \phi _{bev} \right) , z_R=z,
\end{equation}
and it can be projected to the camera frame using extrinsic parameters:
\begin{equation}
    \label{eq:ex}
    \left( \begin{array}{c}
	x_C\\
	y_C\\
	z_C\\
    \end{array} \right) =R\left( \begin{array}{c}
    	x_R\\
    	y_R\\
    	z_R\\
    \end{array} \right) +T=\left( \begin{array}{c}
    	a_1r_{bev}\cos \phi_{bev}+b_1r_{bev}\sin \phi_{bev}+c_1z+d_1\\
    	a_2r_{bev}\cos \phi_{bev}+b_2r_{bev}\sin \phi_{bev}+c_2z+d_2\\
    	a_3r_{bev}\cos \phi_{bev}+b_3r_{bev}\sin \phi_{bev}+c_3z+d_3\\
    \end{array} \right). 
\end{equation}
Using the intrinsic parameters, the camera coordinate $(x_C, y_C, z_C)$ can be correlated with image pixel position $(x_I, y_I)$ using:
\begin{equation}
    \label{eq:in}
    \frac{x_I-u_0}{f_x}=\frac{x_C}{z_C},\frac{y_I-v_0}{f_y}=\frac{y_C}{z_C},
\end{equation}
where $f_x$, $f_y$, $u_0$, and $v_0$ are intrinsic parameters. Our goal is to find a situation that the pillar is projected as a column on the image plane. Under this condition, $x_I$ should be irrelevant with $z$, i.e. in the equation below:
\begin{equation}
    \label{eq:col_org}
    \frac{x_I-u_0}{f_x}=\frac{x_C}{z_C}=\frac{a_1r_{bev}\cos \phi_{bev} +b_1r_{bev}\sin \phi_{bev} +c_1z+d_1}{a_3r_{bev}\cos \phi_{bev} +b_3r_{bev}\sin \phi_{bev} +c_3z+d_3}.
\end{equation}
The coefficients of z should be 0, which means  by combining the relationship between rotation matrix $R$ with roll $\alpha$, pitch $\beta$, and yaw $\gamma$ \cite{murray1994mathematical}, we can derive:
\begin{equation}
    \label{eq:c1&c3}
    \left\{ \begin{array}{l}
    	c_1=\sin \gamma \sin \alpha +\cos \gamma \sin \beta \cos \alpha =0\\
    	c_3=\cos \beta \cos \alpha =0.\\
    \end{array} \right. 
\end{equation}
Considering second row of \cref{eq:c1&c3}, there are two solutions  $\beta=\pm\frac{\pi}{2}$ or $\alpha=\pm\frac{\pi}{2}$. Considering the first solution $\beta=\pm\frac{\pi}{2}$, the first row of \cref{eq:c1&c3} is transformed to:
\begin{equation}
    \sin \gamma \sin \alpha \pm \cos \gamma \cos \alpha =0,
\end{equation}
which means:
\begin{equation}
    \cos \left( \gamma \mp \alpha \right) =0.
\end{equation}
Thus we have:
\begin{equation}
    \begin{aligned}
        \beta &=\frac{\pi}{2}, \gamma =\alpha \pm \frac{\pi}{2}, \alpha \in \left[ -\pi ,\pi \right] \,\, ,\\
	or, \,\,\beta &=-\frac{\pi}{2},\gamma =-\alpha \pm \frac{\pi}{2}, \alpha \in \left[ -\pi ,\pi \right].\\
    \end{aligned}
\end{equation}
For another solution $\alpha=\pm\frac{\pi}{2}$, the first row of \cref{eq:c1&c3} is transformed to:
\begin{equation}
    \sin \gamma \sin \alpha +\cos \gamma \sin \beta \cos \alpha =\pm \sin \gamma =0.
\end{equation}
Thus we have:
\begin{equation}
    \alpha =\pm \frac{\pi}{2}, \gamma =0 \,\,or\,\,\pi , \beta \in \left[ -\pi ,\pi \right].\\
\end{equation}
As a result, the final solution is:
\begin{equation}
    \label{eq:colsolu}
    \begin{aligned}
        \beta &=\frac{\pi}{2}, \gamma =\alpha \pm \frac{\pi}{2}, \alpha \in \left[ -\pi ,\pi \right] ,\\
    	or,\, \beta &=-\frac{\pi}{2}, \gamma =-\alpha \pm \frac{\pi}{2}, \alpha \in \left[ -\pi ,\pi \right],\\
    	or,\, \alpha &=\pm \frac{\pi}{2}, \gamma =0 \,\,or\,\,\pi , \beta \in \left[ -\pi ,\pi \right].\\
    \end{aligned}
\end{equation}

% \textbf{If the slope of the projected line is $0$}, the projected line is indeed a row, which means $y_I$ is irrelevant with $z$, i.e. in the equation below:
% \begin{equation}
%     \frac{y_I-v_0}{f_y}=\frac{y_C}{z_C}=\frac{a_2r_{bev}\cos \phi_{bev} +b_2r_{bev}\sin \phi_{bev} +c_2z+d_2}{a_3r_{bev}\cos \phi_{bev} +b_3r_{bev}\sin \phi_{bev} +c_3z+d_3}
% \end{equation}
% The coefficients of z are 0, so similarly, we have that:
% \begin{equation}
%     \begin{cases}
%     	c_2=-\cos \gamma \sin \alpha +\sin \gamma \sin \beta \cos \alpha =0\\
%     	c_3=\cos \beta \cos \alpha =0\\
%     \end{cases}
% \end{equation}
% Solving this equation set, we can get the solution:
% \begin{equation}
%     \begin{cases}
%     	\beta =\frac{\pi}{2}, \gamma =\alpha \,\,or\,\,\alpha +\pi \,\,, \alpha \in \left[ -\pi ,\pi \right]\\
%     	\beta =-\frac{\pi}{2}, \gamma =-\alpha \,\,or\,-\alpha +\pi \,\,, \alpha \in \left[ -\pi ,\pi \right]\\
%     	\alpha =\pm \frac{\pi}{2},\gamma =\pm \frac{\pi}{2}, \beta \in \left[ -\pi ,\pi \right]\\
%     \end{cases}
% \end{equation}

% \textbf{For other conditions}, the slope of the projected is irrelevant with $z$. Combining \cref{eq:ex} and \cref{eq:in}, we have that:
% \begin{equation}
%     \frac{y_I-v_0}{f_y}\frac{f_x}{x_I-u_0}=\frac{y_C}{x_C}=\frac{a_2r_{bev}\cos \phi_{bev} +b_2r_{bev}\sin \phi_{bev} +c_2z+d_2}{a_1r_{bev}\cos \phi_{bev} +b_1r_{bev}\sin \phi_{bev} +c_1z+d_1}
% \end{equation}
% and we can consequently derive that:
% \begin{equation}
%     y_I=v_0+\frac{a_2r_{bev}\cos \phi_{bev} +b_2r_{bev}\sin \phi_{bev} +c_2z+d_2}{a_1r_{bev}\cos \phi_{bev} +b_1r_{bev}\sin \phi_{bev} +c_1z+d_1}\frac{f_y}{f_x}\left( x_I-u_0 \right) 
% \end{equation}
% the slope should also be irrelevant with $z$, thus the coefficients of z are 0. Similarly, we have that:
% \begin{equation}
%     \begin{cases}
%     	c_1=\sin \gamma \sin \alpha +\cos \gamma \sin \beta \cos \alpha =0\\
%     	c_2=-\cos \gamma \sin \alpha +\sin \gamma \sin \beta \cos \alpha =0\\
%     \end{cases}
% \end{equation}
% Solving this equation set, we can get the solution:
% \begin{equation}
%     \alpha =0\,\, or\,\,\pi , \beta =0\,\,or\,\,\pi , \gamma \in \left[ -\pi ,\pi \right] 
% \end{equation}
\begin{wrapfigure}{r}{0.4\textwidth}
\centering
\vspace{-10pt}
\includegraphics[width=0.35\textwidth]{Figures/Coord.pdf}
\caption{Illustration of coordinate system transformation.}
\label{fig:coord}
\vspace{-20pt}
\end{wrapfigure}

In standard ADS, the LiDAR or radar coordinate system usually has a z-axis pointing up, while the camera coordinate system has a y-axis pointing up or down. So a widely adopted practice first exchanges the y and z axes, which means a roll $\alpha = \pm \frac{\pi}{2}$. After that, a pitch $\beta$ around the vertical y-axis is executed, while further rotation around the z-axis is not required, as shown in \cref{fig:coord}. In other words, the roll $\beta$ can be any value between $-\pi$ and $\pi$, while yaw $\gamma$ is set to 0. This is exactly the situation of the third solution of \cref{eq:colsolu}. And under this condition, we have:
\begin{equation}
    R=\left( \begin{matrix}
    	\cos \beta&		\pm \sin \beta&		0\\
    	0&		0&		\mp 1\\
    	-\sin \beta&		\pm \cos \beta&		0\\
    \end{matrix} \right) , T=\left( \begin{array}{c}
    	d_1\\
    	d_2\\
    	d_3\\
    \end{array} \right) .
\end{equation}
Thus, using \cref{eq:ex} and \cref{eq:col_org}, we can get the expression of column index $x_I$. If $\alpha =\frac{\pi}{2}$, we have:
\begin{equation}
    x_I=u_0+f_x\frac{r_{bev}\cos \left( \beta -\phi _{bev} \right) +d_1}{-r_{bev}\sin \left( \beta -\phi _{bev} \right) +d_3}.
\end{equation}
If $\alpha =-\frac{\pi}{2}$, we have:
\begin{equation}
	x_I=u_0+f_x\frac{r_{bev}\cos \left( \beta +\phi _{bev} \right) +d_1}{-r_{bev}\sin \left( \beta +\phi _{bev} \right) +d_3}.
\end{equation}
For RADIal, the rotation matrix from the radar coordinate system to the camera coordinate system is:
\begin{equation}
    R=\left( \begin{matrix}
	0.0465&		-0.9989&		-0.0051\\
	0.0476&		-0.0029&		0.9989\\
	-0.9978&		-0.0467&		0.0474\\
    \end{matrix} \right), 
\end{equation}
which is the approximation of $(\alpha, \beta, \gamma)=(-\pi/2, \pi/2, 0)$. And thus we approximately have:
\begin{equation}
    x_I \approx u_0+f_x\frac{-r_{bev}\sin \phi _{bev}+d_1}{-r_{bev}\cos \phi _{bev}+d_3}.
\end{equation}
It can be inferred that $x_I$ is almost irrelevant to $z$, which means one pillar in the polar coordinate of radar corresponds to a column in the image.

\section{Visualization and Dataset Statistics}
\label{sec:data}
\begin{figure}[t]
\centering
\includegraphics[width=0.99\columnwidth]{Figures/Vis.pdf}
\caption{Visualization of ground truths and predictions from RT and image fusion. The ground truth bounding boxes are in \textcolor[rgb]{1,0,1}{pink}, while the predicted bounding boxes are in \textcolor[rgb]{0,0.5,0}{green} with the confidence score on its upper right. The LiDAR points and the radar points are respectively in \textcolor[rgb]{0,0,1}{blue} and \textcolor[rgb]{1,0,0}{red}. The rear edge of each car is in \textcolor[rgb]{0,0.75,0.75}{cyan}. }
\label{fig:vis}
\end{figure}
To better illustrate the performance of our method, we visualize the predictions and ground truths in \cref{fig:vis}. As can be seen from the cases in the first and the second column, our method can accurately predict the position of vehicles. But there are several cases in which the accurate prediction does not get high confidence, as shown in the upper case in the third column. On the other hand, the orientation estimation error may be significant when the yaw of the vehicle is large, shown in the inferior case in the third column. The main reason is that the samples with large yaw are relatively rare in the dataset, as shown in \cref{fig:data_stat} (b) and (c).

\begin{figure}[t]
\centering
\includegraphics[width=0.99\columnwidth]{Figures/DataStatistics.pdf}
\caption{Statistics of RADIal dataset. Image (a) corresponds to sample distribution over range, while images (b) and (c) correspond to yaw distribution over the range of train and test data splits.}
\label{fig:data_stat}
\end{figure}
As shown in \cref{fig:data_stat} (a), the samples of test data are rather rare within 30 meters and out of 80 meters. To comprehensively explore the detection performance of objects, we divide the range into 0-50m and 50-100m, which correspond to short-range and long-range detection performance respectively.

%Thus a vastly adopted range interval of 5-30m, 30-50m, and 50-80m would lead to unrepresentative short-range performance. We adopt a more suitable division, 0-50m and 50-100m, so as to more comprehensively explore the detection performance of objects.



\section{Complementary property of radar and camera}
\label{sec:R&C}
\begin{table}
  \caption{LET-BEV-AP results with different longitudinal tolerance $T_l$. The performances of different modality combinations of our algorithm on RADIal Dataset test split are presented, using refined 3D bounding box annotations. C, L, and RT respectively refer to the camera, LiDAR, and range-time data. The results with LiDAR are on gray background.}
  \label{tab:let-bev}
  \centering
  \resizebox{0.99\textwidth}{!}{%
  \begin{tabular}{lllllllll}
    \toprule
    \multicolumn{3}{c}{Modality} & \multicolumn{3}{c}{$T_l=0.1$, LET-BEV-AP@0.7($\%$)$\uparrow$}&\multicolumn{3}{c}{ $T_l=0.3$, LET-BEV-AP@0.7($\%$)$\uparrow$}\\
    \cmidrule(r){1-3} \cmidrule(r){4-6} \cmidrule(r){7-9}
    C & RT & L & Overall & 0 - 50m & 50 - 100m & Overall & 0 - 50m & 50 - 100m \\
    \midrule
    \checkmark & & & 56.92$\pm$3.91 & 78.98$\pm$1.41 & 36.20$\pm$5.81 & 81.36$\pm$1.15 & 83.30$\pm$2.01 & 77.00$\pm$0.43\\
     & \checkmark & & 55.04$\pm$1.25 & 68.56$\pm$4.11 & 52.30$\pm$1.82 & 55.34$\pm$1.91 & 69.79$\pm$4.59 & 51.02$\pm$0.07\\
    \rowcolor{gray!20} & & \checkmark & 86.07$\pm$0.44 & 88.55$\pm$0.79 & 93.17$\pm$0.10 & 86.41$\pm$0.47 & 89.72$\pm$0.03 & 93.22$\pm$0.04\\
    \midrule
    \checkmark & \checkmark & & 88.86$\pm$0.62 & 92.81$\pm$1.37 & 94.81$\pm$0.52 & 88.56$\pm$0.53 & 92.58$\pm$0.70 & 94.57$\pm$0.29\\
    %\rowcolor{gray!20}
    %\checkmark & & & \checkmark & \checkmark & 86.53$\pm$0.05 & 87.98$\pm$1.11 & 95.08$\pm$0.47 & 88.35$\pm$0.24 & 91.30$\pm$0.42 & 96.19$\pm$0.58 \\
    \bottomrule
  \end{tabular}
  }
\end{table}

\begin{table}
  \caption{Recall with different IoU thresholds. The performances of different modality combinations of our algorithm on RADIal Dataset test split are presented, using refined 3D bounding box annotations. C, L, and RT respectively refer to the camera, LiDAR, and range-time data. The results with LiDAR are on gray background.}
  \label{tab:recall}
  \centering
  \resizebox{0.99\textwidth}{!}{%
  \begin{tabular}{lllllllll}
    \toprule
    \multicolumn{3}{c}{Modality} & \multicolumn{3}{c}{BEV recall@0.7($\%$)$\uparrow$}&\multicolumn{3}{c}{BEV recall@0.3($\%$)$\uparrow$}\\
    \cmidrule(r){1-3} \cmidrule(r){4-6} \cmidrule(r){7-9}
    C & RT & L & Overall & 0 - 50m & 50 - 100m & Overall & 0 - 50m & 50 - 100m \\
    \midrule
     & \checkmark & & 62.73$\pm$1.24 & 73.89$\pm$2.11 & 61.21$\pm$0.82 & 86.27$\pm$0.43 & 92.13$\pm$0.71 & 93.40$\pm$0.54\\
    \rowcolor{gray!20} & & \checkmark & 86.38$\pm$0.00 & 89.11$\pm$0.08 & 93.35$\pm$0.08 & 91.40$\pm$0.08 & 96.13$\pm$0.17 & 96.95$\pm$0.16\\
    \midrule
    \checkmark & \checkmark & & 86.18$\pm$0.13 & 89.13$\pm$0.6 & 92.53$\pm$0.56 & 91.78$\pm$0.85 & 95.82$\pm$0.50 & 97.67$\pm$1.05\\
    \bottomrule
  \end{tabular}
  }
\end{table}


To highlight the complementary nature of radar and camera properties, we investigated the performance of LET-BEV-AP with varying longitudinal tolerance ($T_l$), as presented in Table \ref{tab:let-bev}. Notably, when using a larger $T_l$ of 0.3, the camera's performance experiences a significant improvement. This suggests that the relatively lower performance of long-range LET-BEV-AP under $T_l$ of 0.1 primarily stems from depth errors. By reducing the impact of longitudinal estimation, the camera's exceptional angular perception accuracy becomes more pronounced. Conversely, the LET-BEV-AP performance of the radar-only variant remains relatively unchanged. This finding indicates that the radar's depth estimation is quite accurate and minimally affected by the value of $T_l$. Similarly, the highly accurate LiDAR-only variant and camera and RT fusion variant don't suffer from performance fluctuation as well, which supports our conclusion.

To further investigate the primary factor affecting radar performance, we conducted a comparison of BEV recall at IoU thresholds of 0.7 and 0.3, as outlined in Table \ref{tab:recall}. It can be deduced that by using a less stringent IoU threshold, the recall of the RT-only variant experiences a significant increase. This result suggests that the RT-only variant's limitation mainly lies in its inferior angular localization ability. But by combining the strengths of camera and radar modalities, the model can leverage the advantages of both modalities, leading to a significant performance boost. 

\section{More experimental results}
\label{sec:detail}
\begin{table}
  \caption{BEV detection performances of different modality combinations of our algorithm on RADIal Dataset test split. Refined 3D bounding box annotations are applied. C, L, RD, RT, RA, RP respectively refer to the camera, LiDAR, range-Doppler spectrum, range-time data, range-azimuth map, and radar point cloud. The best result without LiDAR of each metric are in \textbf{bold}, and the results with LiDAR are on gray background.}
  \label{tab:RD}
  \centering
  \resizebox{0.99\textwidth}{!}{%
  \begin{tabular}{llllllllllll}
    \toprule
    \multicolumn{6}{c}{Modality} & \multicolumn{3}{c}{BEV AP@0.7($\%$)$\uparrow$}&\multicolumn{3}{c}{LET-BEV-AP@0.7($\%$)$\uparrow$}\\
    \cmidrule(r){1-6} \cmidrule(r){7-9} \cmidrule(r){10-12}
    C & RT & RD & RA & RP & L & Overall & 0 - 50m & 50 - 100m & Overall & 0 - 50m & 50 - 100m \\
    \midrule
    \checkmark & & & & & & 10.07$\pm$1.10 & 21.68$\pm$3.11 & 2.21$\pm$0.59 & 56.92$\pm$3.91 & \textbf{78.98$\pm$1.41} & 36.20$\pm$5.81 \\
    & \checkmark & & & & & 48.26$\pm$0.92 & 62.33$\pm$4.00 & 45.05$\pm$0.98 & 55.04$\pm$1.25 & 68.56$\pm$4.11 & 52.30$\pm$1.82 \\
    & & \checkmark  & & & & 47.34$\pm$0.73 & 59.31$\pm$1.64 & 42.53$\pm$1.98 & 54.96$\pm$0.67 & 67.02$\pm$1.67 & 50.59$\pm$0.26 \\
    & & & \checkmark & & & 50.67$\pm$1.03 & 65.05$\pm$1.59 & 42.98$\pm$0.51 & 58.53$\pm$0.13 & 72.95$\pm$0.78 & 51.41$\pm$0.54 \\
    & & & & \checkmark & & \textbf{53.55$\pm$0.70} & \textbf{66.19$\pm$1.72} & \textbf{47.41$\pm$1.06} & \textbf{62.59$\pm$1.14} & 76.45$\pm$2.06 & \textbf{56.73$\pm$1.33} \\ \rowcolor{gray!20}
    & & & & & \checkmark & 84.47$\pm$0.15 & 86.92$\pm$0.61 & 91.91$\pm$0.13 & 86.07$\pm$0.44 & 88.55$\pm$0.79 & 93.17$\pm$0.10 \\
    \midrule
    \checkmark & \checkmark & & & & & \textbf{84.92$\pm$0.98} & 87.56$\pm$1.58 & 91.06$\pm$1.18 & 88.86$\pm$0.62 & 92.81$\pm$1.37 & 94.81$\pm$0.52 \\
    \checkmark & & \checkmark & & & & 83.31$\pm$0.39 & 87.26$\pm$0.56 & 89.16$\pm$0.44 & 88.24$\pm$0.06 & 92.18$\pm$0.43 & 93.26$\pm$0.73 \\
    \checkmark & & & \checkmark & & & 84.77$\pm$0.65& \textbf{87.93$\pm$0.60} & \textbf{91.48$\pm$0.28} & \textbf{89.54$\pm$0.54} & \textbf{93.83$\pm$0.56} & \textbf{94.87$\pm$0.58} \\
    \checkmark & & & & \checkmark & & 82.35$\pm$0.93 & 86.97$\pm$1.01 & 86.39$\pm$0.74 & 88.35$\pm$0.78 & 93.07$\pm$0.80 & 92.77$\pm$0.69 \\ \rowcolor{gray!20}
    \checkmark & & & & & \checkmark & 86.35$\pm$1.15 & 88.81$\pm$1.40 & 94.25$\pm$1.68 & 88.44$\pm$0.79 & 91.63$\pm$1.34 & 95.31$\pm$1.28 \\ 
    %\rowcolor{gray!20}
    %\checkmark & & & \checkmark & \checkmark & 86.53$\pm$0.05 & 87.98$\pm$1.11 & 95.08$\pm$0.47 & 88.35$\pm$0.24 & 91.30$\pm$0.42 & 96.19$\pm$0.58 \\
    \bottomrule
  \end{tabular}
  }
\end{table}
Referring to Table \ref{tab:RD}, we have included the detection performance when our model consumes the radar-Doppler spectrum as input. In the case of the single modality version, the performance discrepancy between RT and RD remains within the margin of error. When considering the fusion of image data, the performance of RD slightly lags behind that of RT. These findings suggest that the integration of image data significantly mitigates the importance of conventional radar signal processing in the accurate radar-based detection.

\begin{table}
  \caption{3D detection performances on RADIal Dataset test split with refined 3D ground-truth bounding box. C, L, and RT respectively refer to camera, LiDAR, and radar-time data. The best result of each metric is in \textbf{bold}.}
  \label{tab:+-3DmAP}
  \centering
  \resizebox{0.99\textwidth}{!}{%
  \begin{tabular}{lllllll}
    \toprule
    & \multicolumn{3}{c}{3D AP@0.5($\%$)$\uparrow$}&\multicolumn{3}{c}{Average Error@0.5$\downarrow$}\\
    \cmidrule(r){2-4} \cmidrule(r){5-7}
     Modality & Overall & 0 - 50m & 50 - 100m & ATE & ASE & AOE\\
    \midrule
    L & 62.58$\pm$0.11 & 80.65$\pm$0.61 & 53.31$\pm$0.96 & \textbf{0.247$\pm$0.004} & \textbf{0.172$\pm$0.001} & 0.026$\pm$0.001 \\
    L\&C & \textbf{68.23$\pm$0.13} & \textbf{82.50$\pm$2.25} & \textbf{61.59$\pm$0.05} & 0.255$\pm$0.016 & 0.203$\pm$0.023 & 0.026$\pm$0.006 \\
    RT\&C & 41.27$\pm$1.06 & 64.42$\pm$5.31 & 28.19$\pm$1.75 & 0.318$\pm$0.008 & 0.192$\pm$0.014 & \textbf{0.023$\pm$0.002} \\
    \bottomrule
  \end{tabular}
  }
\end{table}
Furthermore, we offered averaged 3D detection results, as listed in \cref{tab:+-3DmAP}. As can be observed, the performance of radar and image fusion still lags far from LiDAR-based methods. The primary limitation can be attributed to imperfect z localization, resulting in relatively high Average Localization Error (ATE). As mentioned in Section 5.5, the inferior performance is mainly due to coarse LiDAR annotation and inferior radar elevation resolution. The low elevation distinguishing power of LiDAR makes annotation error much worse at long range. As a result, both LiDAR-based and radar-based methods experience a significant drop in 3D AP within the 50-100m interval. This emphasizes the pressing need for a dataset of higher quality that enables better exploration of radar data usage.
